Open Set Wireless Standard Classification Using Convolutional Neural Networks

In congested electromagnetic environments, cognitive radios require knowledge about other emitters in order to optimize their dynamic spectrum access strategy. Deep learning classification algorithms have been used to recognize the wireless signal standards of emitters with high accuracy, but are limited to classifying signal classes that appear in their training set. This diminishes the performance of deep learning classifiers deployed in the field because they cannot accurately identify signals from classes outside of the training set. In this paper, a convolution neural network based open set classifier is proposed with the ability to detect if signals are not from known classes by thresholding the output sigmoid activation. The open set classifier was trained on 4G LTE, 5G NR, IEEE 802.11ax, Bluetooth Low Energy 5.0, and Narrowband Internet-of-Things signals impaired with Rayleigh or Rician fading, AWGN, frequency offsets, and in-phase/quadrature imbalances. Then, the classifier was tested on OFDM, SC-FDMA, SC, AM, and FM signals, which did not appear in the training set classes. The closed set classifier achieves an average accuracy of 94.5% for known signals with SNR's greater than 0 dB, but by design, has a 0% accuracy detecting signals from unknown classes. On the other hand, the open set classifier retains an 86% accuracy for known signal classes, but can detect 95.5% of signals from unknown classes with SNR's greater than 0 dB.

==> sections/tables.tex <==
\begin{table}[H]
    \caption{4G LTE Downlink Signal Parameters}
    \label{tab:4g_parameters}
    \begin{tabular}{|| m{3.5cm} | m{4.3cm}||}
        \hline
        Parameter & Values\\
        \hline\hline
        Waveform & OFDMA\\
        \hline
        Subcarrier Spacing & 15 kHz\\
        \hline
        Bandwidth & 1.4, 3, 5, 10, 15, 20 MHz\\
        \hline
        Cyclic Prefix & Normal, Extended\\
        \hline
        PHICH Group Size & Sixth, One, Two\\
        \hline
        PDCCH Aggregation & 1, 3\\
        \hline
        PDSCH Resource Blocks & Random\\
        \hline
        PDSCH Modulation & QPSK, 16 QAM, 64 QAM, 256 QAM\\
        \hline
        PDSCH Usage & 1, 25, 50, 75, 100 \%\\
        \hline
        Duplex Mode & FDD\\
        \hline
    \end{tabular}
\end{table}

\begin{table}[H]
    \caption{5G NR Downlink Signal Parameters}
    \label{tab:5g_parameters}
    \begin{tabular}{|| m{3.5cm} | m{4.3cm}||}
        \hline
        Parameter & Values\\
        \hline\hline
        Waveform & OFDMA\\
        \hline
        Subcarrier Spacing & 15, 30 kHz\\
        \hline
        Bandwidth (15 kHz Spacing) & 5, 10, 15, 20, 25, 40, 50 MHz\\
        \hline
        Bandwidth (30 kHz Spacing) & 10, 20, 30, 50, 80, 100 MHz\\
        \hline
        Frequency Range & FR1 -- $<$3 GHz and 3-6 GHz\\
        \hline    
        SSB Period & 20 ms\\
        \hline
        PDCCH Aggregation & 1, 2\\
        \hline
        CORESET Postion & Random\\
        \hline
        PDSCH Resource Blocks & Random\\
        \hline
        PDSCH Modulation & 16 QAM, 64 QAM, 256 QAM\\
        \hline
        PDSCH Usage & 1, 25, 50, 75, 100 \%\\
        \hline
        % PDSCH PTRS & Enabled\\
        % \hline
        % Additional PDSCH DMRS & 0\\
        % \hline
        Duplex Mode & FDD\\
        \hline
    \end{tabular}
\end{table}

\begin{table}[H]
    \caption{4G LTE Uplink Signal Parameters}
    \label{tab:4gUp_parameters}
    \begin{tabular}{|| m{3.5cm} | m{4.3cm}||}
        \hline
        Parameter & Values\\
        \hline\hline
        Waveform & SC-FDMA\\
        \hline
        Bandwidth & 1.4, 3, 5, 10, 15, 20 MHz\\
        \hline
        PUSCH Modulation & QPSK, 16 QAM, 64 QAM\\
        \hline
        PUSCH Usage & 1, 25, 50, 75, 100 \%\\
        \hline
        Number of active UE & 1-8\\
        \hline
        PUCCH Format & 1\\
        \hline
        PUSCH Resource Blocks & Random\\
        \hline
        PRACH Subframes & Random\\
        \hline
        Duplex Mode & FDD\\
        \hline
    \end{tabular}
\end{table}

\begin{table}[H]
    \caption{5G NR Uplink Signal Parameters}
    \label{tab:5gUp_parameters}
    \begin{tabular}{|| m{3.5cm} | m{4.3cm}||}
        \hline
        Parameter & Values\\
        \hline\hline
        Waveform & OFDM, SC-FDMA\\
        \hline
        Subcarrier Spacing & 15, 30 kHz\\
        \hline
        Bandwidth (15 kHz Spacing) & 5, 10, 15, 20, 25, 40, 50 MHz\\
        \hline
        Bandwidth (30 kHz Spacing) & 10, 20, 30, 50, 80, 100 MHz\\
        \hline
        Frequency Range & FR1\\
        \hline
        PUSCH Modulation & $\frac{\pi}{2}$-BPSK, QPSK, 16 QAM, 64 QAM\\
        \hline
        PUSCH Usage & 1, 25, 50, 75, 100 \%\\
        \hline
        Number of active UE & 1-14\\
        \hline
        PUCCH Format & 0, 1, 2, 3, 4\\
        \hline
        PUSCH Resource Blocks & Random\\
        \hline
        PRACH Subframes & Random\\
        \hline
        Duplex Mode & FDD\\
        \hline
    \end{tabular}
\end{table}

\begin{table}[H]
    \caption{IEEE 802.11ax (WiFi 6) Signal Parameters}
    \label{tab:wifi_parameters}
    \begin{tabular}{|| m{3.5cm} | m{4.3cm}||}
        \hline
        Parameter & Values\\
        \hline\hline
        Waveform & OFDMA\\
        \hline
        Subcarrier Spacing & 78.125 kHz\\
        \hline
        Bandwidth & 20, 40, 80 MHz\\
        \hline
        MCS & 0 -- 11\\
        \hline
        Usage & 1, 25, 50, 75, 100 \%\\
        \hline
        Packet Formats & Single-user, Extended-range single-user, Multi-user, Trigger-based \\
        \hline
        Packet duration & No Data Packet (NDP) -- max duration (5.4 ms)\\
        \hline
        Guard interval & 0.8, 1.6, 3.2 $\mu s$\\
        \hline
        Channel coding & LDPC, BCC\\
        \hline
        Multiuser Allocation Modes & 0 -- 15\\
        \hline
        Duplex Mode & TDD\\
        \hline
    \end{tabular}
\end{table}

\begin{table}[H]
    \caption{Bluetooth Low Energy (BLE) 5.0 Signal Parameters}
    \label{tab:BLE_parameters}
    \begin{tabular}{|| m{3.5cm} | m{4.3cm}||}
        \hline
        Parameter & Values\\
        \hline\hline
        Waveform & FHSS\\
        \hline
        Bandwidth & 2 MHz\\
        \hline
        Symbol rate & 1, 2 MBd\\
        \hline
        Modulation & GFSK\\
        \hline
        PHY & LE 2M, LE 1M, LE Coded 500K, LE Coded 125K\\
        \hline
        Advertisers & 1 -- 6\\
        \hline
        Active connections & 1 -- 8\\
        \hline
        Devices paired & 0 -- 1\\
        \hline
        Scan requests & 0 -- 1\\
        \hline
        Duplex Mode & TDD\\
        \hline
    \end{tabular}
\end{table}


\begin{table}[H]
    \caption{Signal Parameters}
    \label{tab:signal_parameters}
    \begin{tabular}{|| m{1.2cm} | m{1.1cm} | m{1.1cm} | m{0.8cm} | m{0.8cm} | m{0.8cm} | m{0.8cm}||}
        \hline
        Parameter & 4G Down & 5G Down & 4G Up & 5G Up & WiFi & BLE\\
        \hline\hline
        Waveform & OFDM & OFDM & SC-FDMA & OFDM, SC-FDMA & OFDM & FHSS\\
        \hline
        Subcarrier Spacing (kHz) & 15 & 15, 30 & -- & 15, 30 & 78.125 & --\\
        \hline
        Resource Grid Usage (\%) & 1--100 & 1--100 & 1--100 & 1--100 & -- & -- \\ 
        \hline
        Bandwidth (MHz) & 1.4--20 & 5--100 & 1.4--20 & 5--100 & 20--80 & 2\\
        \hline
        Modulation Order & 4--256 & 16--64 & 4--64 & 4--64 & 2--1024 & 2 (GFSK)\\
        \hline
        Devices & 1 & 1 & 1--8 & 1--14 & 1--9 & 1--14\\
        \hline 
        Duplex Mode & FDD & FDD & FDD & FDD & TDD & TDD\\
        \hline
    \end{tabular}
\end{table}

\begin{table}[H]
    \caption{Signal Parameters}
    \label{tab:signal_parameters}
    \begin{tabular}{|| m{1.6cm} | m{1.2cm} | m{1.2cm} | m{1.4cm} | m{1.4cm} ||}
        \hline
        Parameter & 4G Down & 5G Down & 4G Up & 5G Up\\
        \hline\hline
        Waveform & OFDM & OFDM & SC-FDMA & OFDM, SC-FDMA\\
        \hline
        Subcarrier Spacing & 15 kHz& 15, 30 kHz& -- & 15, 30 kHz\\
        \hline
        Resource Grid Usage & 1--100 \% & 1--100 \% & 1--100 \% & 1--100 \%\\ 
        \hline
        Bandwidth (MHz) & 1.4--20 & 5--100 & 1.4--20 & 5--100\\
        \hline
        Modulation Order & 4--256 & 16--64 & 4--64 & 4--64\\
        \hline
        Devices & 1 & 1 & 1--8 & 1--14\\
        \hline 
        Duplex Mode & FDD & FDD & FDD & FDD\\
        \hline
    \end{tabular}
\end{table}

\begin{table}[H]
    \caption{Signal Parameters}
    \label{tab:signal_parameters}
    \begin{tabular}{|| m{1.2cm} | m{1.1cm} | m{1.1cm} | m{0.8cm} | m{0.8cm} | m{0.8cm} | m{0.8cm}||}
        \hline
        Parameter & 4G Down & 5G Down & 4G Up & 5G Up & WiFi & BLE\\
        \hline\hline
        Waveform & OFDM & OFDM & SC-FDMA & OFDM, SC-FDMA & OFDM & FHSS\\
        \hline
        Subcarrier Spacing (kHz) & 15 & 15, 30 & -- & 15, 30 & 78.125 & --\\
        \hline
        Resource Grid Usage (\%) & 1--100 & 1--100 & 1--100 & 1--100 & -- & -- \\ 
        \hline
        Bandwidth (MHz) & 1.4--20 & 5--100 & 1.4--20 & 5--100 & 20--80 & 2\\
        \hline
        Modulation Order & 4--256 & 16--64 & 4--64 & 4--64 & 2--1024 & 2 (GFSK)\\
        \hline
        Devices & 1 & 1 & 1--8 & 1--14 & 1--9 & 1--14\\
        \hline 
        Duplex Mode & FDD & FDD & FDD & FDD & TDD & TDD\\
        \hline
    \end{tabular}
\end{table}
